Scheduled Restart Momentum for Accelerated Stochastic Gradient Descent

Stochastic gradient descent (SGD) with constant momentum and its variants such as Adam are the optimization algorithms of choice for training deep neural networks (DNNs). Since DNN training is incredibly computationally expensive, there is great interest in speeding up the convergence. Nesterov accelerated gradient (NAG) improves the convergence rate of gradient descent (GD) for convex optimization using a specially designed momentum; however, it accumulates error when an inexact gradient is used (such as in SGD), slowing convergence at best and diverging at worst. In this paper, we propose Scheduled Restart SGD (SRSGD), a new NAG-style scheme for training DNNs. SRSGD replaces the constant momentum in SGD by the increasing momentum in NAG but stabilizes the iterations by resetting the momentum to zero according to a schedule. Using a variety of models and benchmarks for image classification, we demonstrate that, in training DNNs, SRSGD significantly improves convergence and generalization; for instance in training ResNet200 for ImageNet classification, SRSGD achieves an error rate of 20.93% vs. the benchmark of 22.13%. These improvements become more significant as the network grows deeper. Furthermore, on both CIFAR and ImageNet, SRSGD reaches similar or even better error rates with significantly fewer training epochs compared to the SGD baseline.

==> preamble.tex <==
% ---------------------------------
%floats and figures
% ---------------------------------

% if you need to pass options to natbib, use, e.g.:
\PassOptionsToPackage{numbers, compress}{natbib}
\usepackage{amsmath}
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
}
\urlstyle{same}
%\usepackage{array}
\usepackage{booktabs} % for professional tables
\usepackage{amsfonts}
\usepackage{bm}
%\usepackage{soul}
%\usepackage{lmodern}
%\usepackage{booktabs}
\usepackage{threeparttable}
%\usepackage{mathtools}
\usepackage{tablefootnote}

%\usepackage{cuted}
\usepackage{lipsum}
\usepackage{comment}

\usepackage{multirow}
\usepackage[usenames, dvipsnames]{color}
\usepackage{amsmath}

\newcommand\xmod[1]{{\textcolor{blue}{#1}}}
\newcommand\zmod[1]{{\textcolor{red}{#1}}}


\usepackage{hyperref}

\usepackage{enumitem}

\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\usepackage{listings}

\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}

\usepackage{listings}
\usepackage{color}

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstset{ %
  backgroundcolor=\color{white},   % choose the background color
  basicstyle=\footnotesize,        % size of fonts used for the code
  breaklines=true,                 % automatic line breaking only at whitespace
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  keywordstyle=\color{blue},       % keyword style
  stringstyle=\color{mymauve},     % string literal style
}

%=======U S E R  D E F I N E D  M A C R O S=======
% ---------------------------------
% User Comments
% ---------------------------------
\usepackage{marginnote}
% \newcommand{\bibhref}[2]{#2}
\usepackage{soul} %text highlighting
\newcommand{\todohl}[1]{{[\hl{#1?}]}}
% \usepackage[disable]{todonotes}
% \usepackage{todonotes}
\usepackage[colorinlistoftodos]{todonotes}
%takes in optional argument
% \newcommand{\tocite}[1]{%
% \textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}
% }


\newcommand{\ignore}[1]{}
\newcommand{\etal}{et al.~}

%version in control in draft mode
\newcommand{\versionString}{\textcolor{red}{draft-mode-[\today\ \currenttime]}}

% ---------------------------------
% Label utils
% ---------------------------------

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it
\newcommand{\figlabel}[1]{\label{fig:#1}}
% \newcommand{\figref}[1]{Fig.    \,\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
% \newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

\newcommand{\tss}{\hspace*{0.66mm}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% space tweaks 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\abovecaptionskip}{0.5mm}
\setlength{\belowcaptionskip}{0mm} 
\setlength{\textfloatsep}{1.5mm}
\setlength{\dbltextfloatsep}{1.5mm}
%\renewcommand{\baselinestretch}{.9945}

\makeatletter
\newenvironment{mcases}[1][l]
 {\let\@ifnextchar\new@ifnextchar
  \left\lbrace
  \def\arraystretch{1.2}%
  \array{@{}l@{\quad}#1@{}}}
 {\endarray\right.}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions for equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/abstract.tex <==
Stochastic gradient descent (SGD) with constant momentum and its variants such as Adam are the optimization algorithms of choice for training deep neural networks (DNNs). Since DNN training is incredibly computationally expensive, there is great interest in speeding up the convergence. Nesterov accelerated gradient (NAG) improves the convergence rate of gradient descent (GD) for convex optimization using a specially designed momentum; however, it accumulates error when an inexact gradient is used (such as in SGD), slowing convergence at best and diverging at worst. In this paper, we propose \emph{Scheduled Restart SGD} (SRSGD), a new NAG-style scheme for training DNNs. SRSGD replaces the constant momentum in SGD by the increasing momentum in NAG but stabilizes the iterations by resetting the momentum to zero according to a schedule. Using a variety of models and benchmarks for image classification, we demonstrate that, in training DNNs, SRSGD significantly improves convergence and generalization; for instance in training ResNet200 for ImageNet classification, SRSGD achieves an error rate of 20.93\% vs.\ the benchmark of 22.13\%. These improvements become more significant as the network grows deeper. Furthermore, on both CIFAR and ImageNet, SRSGD reaches similar or even better error rates with significantly fewer training epochs compared to the SGD baseline.

==> sections/conclusion.tex <==
We propose the Scheduled Restart SGD (SRSGD), with two major changes from the widely used SGD with constant momentum (without ambiguity we call it SGD). First, we replace the momentum in SGD with the increasing momentum in Nesterov accelerated gradient (NAG). Second, we restart the momentum according to a schedule to prevent error accumulation when the stochastic gradient is used. For image classification, SRSGD can significantly improve the accuracy of the trained DNNs. Also, compared to the SGD baseline, SRSGD requires fewer training epochs to reach to the same trained model's accuracy. There are numerous avenues for future work: 1) deriving the optimal restart scheduling and the corresponding convergence rate of SRSGD, 2) integrating the scheduled restart NAG momentum with adaptive learning rate algorithms, e.g. Adam, and 3) integrating SRSGD with optimizers that remove noise on the fly, e.g., Laplacian smoothing SGD \cite{osher2018laplacian}.

==> sections/experiments.tex <==
\renewcommand\arraystretch{1.3}
\setlength{\tabcolsep}{4pt}
\begin{table*}[t!]
\caption{Classification test error (\%) on CIFAR10 using the SGD, %baseline, 
SGD $+$ NM, and SRSGD. We report the results of SRSGD with two different restarting schedules: linear (lin) and exponential (exp). The numbers of iterations after which we restart the momentum in the lin schedule are 30, 60, 90, 120 for the 1st, 2nd, 3rd, and 4th stage. 
%learning rate. 
Those numbers for the exp schedule are 40, 50, 63, 78. We also include the reported 
%baseline 
results from \cite{he2016identity} (in parentheses) in addition to our reproduced results.}\label{tab:cifar10-acc}
%\vspace{2mm}
\centering
\fontsize{6.5pt}{0.65em}\selectfont
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Network & \# Params&SGD (baseline) & SGD$+$NM & SRSGD & SRSGD  & Improve over & Improve over \\
 & & & & (lin) & (exp) & SGD (lin/exp) & SGD$+$NM (lin/exp) \\
\hline
Pre-ResNet-110 &$1.1$M & $5.25 \pm 0.14$ ($6.37$) & $5.24 \pm 0.16$ & \pmb{$4.93 \pm 0.13$} & $5.00 \pm 0.47$ & $\pmb{0.32}/0.25$ & $\pmb{0.31}/0.24$ \\
Pre-ResNet-290 &$3.0$M & $5.05 \pm 0.23$ & $5.04 \pm 0.12$ & \pmb{$4.37 \pm 0.15$} & $4.50 \pm 0.18$ & $\pmb{0.68}/0.55$ & $\pmb{0.67}/0.54$ \\
Pre-ResNet-470 &$4.9$M & $4.92 \pm 0.10$ & $4.97 \pm 0.15$ & \pmb{$4.18 \pm 0.09$} & $4.49 \pm 0.19$ & $\pmb{0.74}/0.43$ & $\pmb{0.79}/0.48$ \\
Pre-ResNet-650 &$6.7$M & $4.87 \pm 0.14$ & $4.80 \pm 0.14$ & \pmb{$4.00 \pm 0.07$} & $4.40 \pm 0.13$ & $\pmb{0.87}/0.47$ & $\pmb{0.80}/0.40$ \\
%Pre-ResNet-830 &$8.6$M & $95.00 \pm 0.23$ & $95.91 \pm 0.10$ & $95.71 \pm 0.13$ & $\pmb{0.91}/0.71$ \\
Pre-ResNet-1001&$10.3$M & $4.84 \pm 0.19$ ($4.92$) & $4.62 \pm 0.14$ & \pmb{$3.87 \pm 0.07$} & $4.13 \pm 0.10$ & $\pmb{0.97}/0.71$ & $\pmb{0.75}/0.49$ \\
\hline
\end{tabular}
\end{table*}
\vskip -0.3cm

We evaluate SRSGD on a variety of DL benchmarks for image classification, including CIFAR10, CIFAR100, and ImageNet. In all experiments, we show the advantage of SRSGD over the widely used and well-calibrated SGD baselines with a constant momentum of $0.9$ and decreasing learning rate at certain epochs, and we denote this optimizer as SGD. We also compare SRSGD with the well-calibrated SGD but switch momentum to the Nesterov momentum 
%(i.e., lookahead momentum) 
of $0.9$, 
and we denoted this optimizer as SGD $+$ NM. 
%we compare SRSGD with SGD with Nesterov momentum of $0.9$, which we denote as SGD $+$ NM. 
We fine tune the SGD/SGD $+$ NM baselines to obtain the best performance, and we then adopt the same set of parameters for training with SRSGD. In the SRSGD experiments, we tune the restart frequencies on small DNNs and apply the tuned restart frequencies to large DNNs. We provide the detailed description of datasets and experimental settings in Appendix~\ref{sec:all-datasets-implementation}.

%%%%%%%%%%%%%%%%%%%%%% CIFAR %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{CIFAR10 and CIFAR100}
\label{sec:cifar-exp}
We summarize our results for CIFAR in Table~\ref{tab:cifar10-acc} and~\ref{tab:cifar100-acc}. We also explore two different restarting frequency schedules for SRSGD: \emph{linear} and \emph{exponential} schedule. These schedules are governed by two parameters: the initial restarting frequency $F_{1}$ and the growth rate $r$. In both scheduling schemes, during training, the restarting frequency at the 1st learning rate stage is set to $F_{1}$. Then the restarting frequency at the $(k+1)$-th learning rate stage is determined by: 
{\small \begin{align}
    F_{k+1} = 
    \begin{cases}
        F_{1} \times r^{k}, &\text{exponential schedule} \\
        F_{1} \times (1 + (r-1) \times k), &\text{linear schedule}.
    \end{cases}\nonumber
\end{align}}
We have conducted a hyper-parameter search for $F_{1}$ and $r$ for both scheduling schemes. For CIFAR10, $(F_{1} = 40, r = 1.25)$ and $(F_{1} = 30, r = 2)$ are good initial restarting frequencies and growth rates for the exponential and linear schedules, respectively. For CIFAR100, those values are $(F_{1} = 45, r = 1.5)$ for the exponential schedule and $(F_{1} = 50, r = 2)$ for the linear schedule. 

\renewcommand\arraystretch{1.3}
\setlength{\tabcolsep}{4pt}
\begin{table*}[t!]
\caption{Classification test error (\%) on CIFAR100 using the SGD, SGD $+$ NM, and SRSGD. We report the results of SRSGD with two different restarting schedules: linear (lin) and exponential (exp). The numbers of iterations after which we restart the momentum in the lin schedule are 50, 100, 150, 200 for the 1st, 2nd, 3rd, and 4th stage. Those numbers for the exp schedule are 45, 68, 101, 152. We also include the reported 
%baseline 
results from \cite{he2016identity} (in parentheses) in addition to our reproduced results.}\label{tab:cifar100-acc}
%\vspace{2mm}
\centering
\fontsize{6.5pt}{0.65em}\selectfont
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Network & \# Params&SGD (baseline) & SGD$+$NM & SRSGD & SRSGD  & Improve over & Improve over \\
 & & & & (lin) & (exp) & SGD (lin/exp) & SGD$+$NM (lin/exp) \\
\hline
Pre-ResNet-110 &$1.2$M & $23.75 \pm 0.20$ & $23.65 \pm 0.36$ &\pmb{$23.49 \pm 0.23$} & $23.50 \pm 0.39$ & $\pmb{0.26}/0.25$ & $\pmb{0.16}/0.15$ \\
Pre-ResNet-290 &$3.0$M & $21.78 \pm 0.21$ & $21.68 \pm 0.21$ & \pmb{$21.49 \pm 0.27$} & $21.58 \pm 0.20$ & $\pmb{0.29}/0.20$ & $\pmb{0.19}/0.10$ \\
Pre-ResNet-470 &$4.9$M & $21.43 \pm 0.30$ & $21.21 \pm 0.30$ & $20.71 \pm 0.32$ & \pmb{$20.64 \pm 0.18$} & $0.72/\pmb{0.79}$ & $0.50/\pmb{0.57}$ \\
Pre-ResNet-650 &$6.7$M & $21.27 \pm 0.14$ & $21.04 \pm 0.38$ &\pmb{$20.36 \pm 0.25$}& $20.41 \pm 0.21$ & $\pmb{0.91}/0.86$ & $\pmb{0.68}/0.63$ \\
Pre-ResNet-1001&$10.4$M & $20.87 \pm 0.20$ ($22.71$) & $20.13 \pm 0.16$ & $19.75 \pm 0.11$ & \pmb{$19.53 \pm 0.19$} & $1.12/\pmb{1.34}$ & $0.38/\pmb{0.60}$\\
\hline
\end{tabular}
\end{table*}

{\bf Improvement in Accuracy Increases with Depth:} We observe that the linear schedule of restart 
%ing frequency 
yields better test error on CIFAR than the exponential schedule for most of the models except for Pre-ResNet-470 and Pre-ResNet-1001 on CIFAR100 (see Table~\ref{tab:cifar10-acc} and~\ref{tab:cifar100-acc}). SRSGD with either linear or exponential restart schedule 
%schedule for restarting frequency 
outperforms the SGD.
%baseline. 
Furthermore, the advantage of SRSGD over SGD is greater for deeper networks. This observation holds strictly when using the linear schedule (see Fig.~\ref{fig:error-vs-depth}) and is overall true when using the exponential schedule with only a few exceptions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[h!]
\centering
\includegraphics[width=1.0\linewidth]{figs/train_loss_vs_epoch_srsgd.pdf}
\vskip -0.4cm
\caption{Training loss vs. training epoch of ResNet models trained with SRSGD (blue) and the SGD baseline with momentum (red).}
\label{fig:train-loss-vs-epoch}
\end{figure}
\end{comment}

{\bf Faster Convergence Reduces the Training Time by Half:} SRSGD also converges faster than SGD. 
%the SGD baseline. 
This is expected since 
%we have observed that 
SRSGD can avoid the error accumulation with inexact oracle and converges faster than SGD + Momentum in our MNIST case study in Section~\ref{section:SRSGD}. For CIFAR, Fig.~\ref{fig:train-loss-vs-epoch} (left) shows that SRSGD yields smaller training loss than SGD during the training. Interestingly, SRSGD converges 
%very 
quickly to good loss values at the 2nd and 3rd stages. 
%learning rate. 
This suggests that \emph{the model can be trained with SRSGD in many fewer epochs compared to SGD} while achieving similar error rate. 

Our numerical results in Table~\ref{tab:cifar-short-train} confirm the hypothesis above. We train Pre-ResNet models with SRSGD \emph{in only 100 epochs}, decreasing the learning rate by a factor of 10 at the 80th, 90th, and 95th epoch while using the same linear schedule for restarting frequency as before with $(F_{1} = 30, r = 2)$ for CIFAR10 and $(F_{1} = 50, r = 2)$ for CIFAR100. We compare the test error of the trained models with those trained by the SGD baseline in 200 epochs. We observe that SRSGD trainings consistently yield lower test errors than SGD except for the case of Pre-ResNet-110 even though \emph{the number of training epochs of our method is only half of the number of training epochs required by SGD}. For Pre-ResNet-110, SRSGD training in 110 epochs with learning rate decreased at the 80th, 90th, and 100th epoch achieves the same error rate as the 200-epoch SGD training on CIFAR10. On CIFAR100, SRSGD training for Pre-ResNet-110 needs 140 epochs with learning rate decreased at the 80th, 100th and 120th epoch to achieve an 0.02\% improvement in error rate over the 200-epoch SGD. %Both 110 and 140 epochs are still much less than 200 epochs. 

\vskip -0.4cm
\renewcommand\arraystretch{1.3}
\setlength{\tabcolsep}{4pt}
\begin{table}[t!]
\caption{Comparison of classification errors on CIFAR10/100 (\%) between SRSGD training \emph{with only 100 epochs} and SGD baseline training with 200 epochs. Using only half the number of training epochs, SRSGD achieves comparable results to SGD.} \label{tab:cifar-short-train}
\vspace{-2.5mm}
\centering
\fontsize{7pt}{0.7em}\selectfont
\begin{tabular}{c|c|c|c|c}
&\multicolumn{2}{c}{CIFAR10} & \multicolumn{2}{c}{CIFAR100}\\
\hline
Network & SRSGD & Improvement & SRSGD & Improvement \\
\hline
Pre-ResNet-110 & $5.43 \pm 0.18$ & $-0.18$ & $23.85 \pm 0.19$ & $-0.10$ \\
Pre-ResNet-290 & $4.83 \pm 0.11$ & $0.22$ & $21.77 \pm 0.43$ & $0.01$ \\
Pre-ResNet-470 & $4.64 \pm 0.17$ & $0.28$ & $21.42 \pm 0.19$ & $0.01$ \\
Pre-ResNet-650 & $4.43 \pm 0.14$ & $0.44 $ & $21.04 \pm 0.20$ & $0.23$  \\
Pre-ResNet-1001 & $4.17 \pm 0.20$ & $0.67$ & $20.27 \pm 0.11$ & $ 0.60$ \\
\hline
Pre-ResNet-110 & $5.25 \pm 0.10$ (110 epochs) & $0.00$ & $23.73 \pm 0.23$ (140 epochs) & $0.02$ \\
\hline
% \hline
\end{tabular}
\end{table}

\begin{comment}
\renewcommand\arraystretch{1.3}
\setlength{\tabcolsep}{4pt}
\begin{table}[t!]
\caption{Comparison of classification errors on CIFAR10/100 (\%) between SRSGD training \emph{with only 100 epochs} and SGD baseline training with 200 epochs. Using only half the number of training epochs, SRSGD achieves comparable results to SGD.} \label{tab:cifar-short-train}
%\vspace{2mm}
\centering
\fontsize{7pt}{0.7em}\selectfont
\begin{tabular}{c|c|c}
\multicolumn{3}{c}{CIFAR10} \\
\hline
Network & SRSGD & Improvement over  \\
& & SGD baseline \\
\hline
Pre-ResNet-110 & $5.43 \pm 0.18$ & $-0.18$ \\
Pre-ResNet-290 & $4.83 \pm 0.11$ & $0.22$ \\
Pre-ResNet-470 & $4.64 \pm 0.17$ & $0.28$ \\
Pre-ResNet-650 & $4.43 \pm 0.14$ & $0.44 $ \\
Pre-ResNet-1001 & $4.17 \pm 0.20$ & $0.67$ \\
\hline
Pre-ResNet-110 & $5.25 \pm 0.10$ (110 epochs) & $0.00$ \\
\hline
\multicolumn{3}{c}{CIFAR100} \\
\hline
Network & SRSGD & Improvement over  \\
& & SGD baseline \\
\hline
Pre-ResNet-110 & $23.85 \pm 0.19$ & $-0.10$ \\
Pre-ResNet-290 & $21.77 \pm 0.43$ & $0.01$ \\
Pre-ResNet-470 & $21.42 \pm 0.19$ & $0.01$ \\
Pre-ResNet-650 & $21.04 \pm 0.20$ & $0.23$ \\
Pre-ResNet-1001 & $20.27 \pm 0.11$ & $ 0.60$ \\
\hline
Pre-ResNet-110 & $23.73 \pm 0.23$ (140 epochs) & $0.02$ \\
\hline
% \hline
\end{tabular}
\end{table}
\end{comment}


%%%%%%%%%%%%%%%%%%%%%% ImageNet %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{ImageNet}
Next we discuss our experimental results on the 1000-way ImageNet classification task \cite{russakovsky2015imagenet}. 
We conduct our 
%ImageNet 
experiments on ResNet-50, 101, 152, and 200 with 5 different seeds. We use the official Pytorch implementation\footnote{Implementation available at \href{https://github.com/pytorch/examples/tree/master/imagenet}{https://github.com/pytorch/examples/tree/master/imagenet}} for all of our ResNet models \cite{paszke2019pytorch}. Following common practice, we train each model for 90 epochs and decrease the learning rate by a factor of 10 at the 30th and 60th epoch. We use an initial learning rate of 0.1, momentum value of 0.9, and weight decay value of 0.0001. Additional details and comparison between SRSGD and SGD $+$ NM are given in Appendix~\ref{appendix:ImageNet:Others}.

We report single crop validation
errors of ResNet models trained with SGD and SRSGD on ImageNet in Table~\ref{tab:imagenet-acc}. In contrast to our CIFAR experiments, we observe that for ResNets trained on ImageNet with SRSGD, linearly decreasing the restarting frequency to 1 at the last learning rate (i.e., after the 60th epoch) helps improve the generalization of the models. Thus, in our experiments, we set the restarting frequency to a linear schedule until epoch 60. From epoch 60 to 90, the restarting frequency is linearly decreased to 1. We use $(F_{1} = 40, r = 2)$. 

\vskip -0.3cm
\renewcommand\arraystretch{1.3}
\setlength{\tabcolsep}{4pt}
\begin{table*}[!ht]
\caption{Single crop validation
errors (\%) on ImageNet of ResNets trained with SGD baseline and SRSGD. We report the results of SRSGD with the increasing restarting frequency in the first two learning rates. In the last learning rate, the restarting frequency is linearly decreased from 70 to 1. For baseline results, we also include the reported single-crop validation errors 
\cite{he@github} (in parentheses).}\label{tab:imagenet-acc}
%\vspace{2mm}
\centering
\fontsize{7pt}{0.7em}\selectfont
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Network & \# Params & \multicolumn{2}{c|}{SGD} & \multicolumn{2}{c|}{SRSGD} & \multicolumn{2}{c}{Improvement} \\
\hline
 &  & top-1 & top-5  & top-1 & top-5  & top-1 & top-5  \\
\hline
ResNet-50 & $25.56$M & $24.11 \pm 0.10$ ($24.70$) & $7.22 \pm 0.14$ ($7.80$) & \pmb{$23.85 \pm 0.09$} & \pmb{$7.10 \pm 0.09$} & $0.26$ & $0.12$ \\
ResNet-101 & $44.55$M & $22.42 \pm 0.03$ ($23.60$) & $6.22 \pm 0.01$ ($7.10$) & \pmb{$22.06 \pm 0.10$} & \pmb{$6.09 \pm 0.07$} & $0.36$ & $0.13$ \\
ResNet-152 & $60.19$M & $22.03 \pm 0.12$ ($23.00$) & $6.04 \pm 0.07$ ($6.70$) & \pmb{$21.46 \pm 0.07$} & \pmb{$5.69 \pm 0.03$} & $0.57$ & $0.35$ \\
ResNet-200 & $64.67$M & $22.13 \pm 0.12$ & $6.00 \pm 0.07$ & \pmb{$20.93 \pm 0.13$} & \pmb{$5.57 \pm 0.05$} & $1.20$ & $0.43$ \\
\hline
\end{tabular}
\end{table*}
\vskip -0.2cm

{\bf Advantage of SRSGD continues to grow with depth:} Similar to the CIFAR experiments, we observe that SRSGD outperforms the SGD baseline for all ResNet models that we study. As shown in Fig.~\ref{fig:error-vs-depth}, \emph{the advantage of SRSGD over SGD grows with network depth}, just as in our CIFAR experiments with Pre-ResNet architectures. 

{\bf Avoiding Overfitting in ResNet-200:} ResNet-200 is an interesting model that demonstrates that \emph{SRSGD is better than the SGD baseline at avoiding overfitting.\footnote{By overfitting, we mean that the model achieves low training error but high test error.}} The ResNet-200 trained with SGD has a top-1 error of 22.18\%, higher than the ResNet-152 trained with SGD, which achieves a top-1 error of 21.9\% (see Table~\ref{tab:imagenet-acc}). As pointed out in \cite{he2016identity}, it is because ResNet-200 suffers from overfitting. The ResNet-200 trained with our SRSGD has a top-1 error of 21.08\%, which is 1.1\% lower than the ResNet-200 trained with the SGD baseline and also lower than the ResNet-152 trained with  both SRSGD and SGD, an improvement by 0.21\% and 0.82\%, respectively.  

\renewcommand\arraystretch{1.3}
\setlength{\tabcolsep}{4pt}
\begin{table}[h!]
\caption{Comparison of single crop validation
errors on ImageNet (\%) between SRSGD training \emph{with fewer epochs} and SGD training with full 90 epochs.}\label{tab:imagenet-short-train}
\vspace{-2mm}
\centering
\fontsize{7pt}{0.7em}\selectfont
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
%Network & SRSGD & Epoch & Improvement  \\
%& & Reduction & over SGD \\
Network & SRSGD & Reduction & Improvement & Network & SRSGD & Reduction & Improvement \\
\hline
ResNet-50 & $24.30 \pm 0.21$ & $10$ & $-0.19$ & ResNet-152 & $21.79 \pm 0.07$ & $15$ & $0.24$ \\
ResNet-101 & $22.32 \pm 0.06$ & $10$ & $0.1$ & ResNet-200 & $21.92 \pm 0.17$ & $30$ & $0.21$ \\
%ResNet-152 & $21.79 \pm 0.07$ & $15$ & $0.24$ \\
%ResNet-200 & $21.92 \pm 0.17$ & $30$ & $0.21$ \\
\hline
% \hline
\end{tabular}
\end{table}

{\bf Training ImageNet in Fewer Number of Epochs: } As in the CIFAR experiments, we note that when training on ImageNet, SRSGD converges faster than SGD at the first and last learning rate while quickly reaching a good loss value at the second learning rate (see Fig.~\ref{fig:train-loss-vs-epoch}). This observation suggests that ResNets can be trained with SRSGD in fewer epochs while still achieving comparable error rates to the same models trained by the SGD baseline using all 90 epochs. We summarize the results in Table~\ref{tab:imagenet-short-train}. On ImageNet, we note that SRSGD helps reduce the number of training epochs for very deep networks (ResNet-101, 152, 200). For smaller networks like ResNet-50, training with fewer epochs slightly decreases the accuracy.  




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Empirical Analysis}\label{section:Empirical-Analysis}

%\subsection{Error Rate vs. Reduction in Epochs}
\paragraph{Error Rate vs. Reduction in Epochs.}
\begin{comment}
\begin{figure}[!t]
\centering
\includegraphics[width=1.0\linewidth]{figs/error_epoch_reduction.pdf}
\vspace{-0.2in}
\caption{Test error vs.\ number of epoch reduction in CIFAR10 and ImageNet training. The dashed lines are test errors of the SGD baseline. For CIFAR, SRSGD training with fewer epochs can achieve comparable results to SRSGD training with full 200 epochs. For ImageNet, training with less epochs slightly decreases the performance of SRSGD but still achieves comparable results to the SGD baseline training.}
\label{fig:error-vs-epoch-reduction}
\end{figure}
\end{comment}

We find that SRSGD training using fewer epochs yield comparable error rate to both the SGD baseline and the SRSGD full training with 200 epochs on CIFAR. We conduct an ablation study to understand the impact of reducing the number of epochs on the final error rate when training with SRSGD on CIFAR10 and ImageNet. In the CIFAR10 experiments, we reduce the number of epochs from 15 to 90 while in the ImageNet experiments, we reduce the number of epochs from 10 to 30.
We summarize our results in Fig.~\ref{fig:error-vs-epoch-reduction} and provide detailed results in Appendix~\ref{sec:error-rate-vs-epoch-reduction-appendix}. For CIFAR10, we can train with 30 epochs less while still maintaining a comparable error rate to the full SRSGD training, and with a better error rate than the SGD baseline. For ImageNet, SRSGD training with fewer epochs decreases the accuracy but still obtains comparable results to the 90-epoch SGD baseline as shown in Table~\ref{tab:imagenet-short-train}.
% \subsubsection{SRSGD on Neural Machine Translation}
\vskip -0.2cm
\begin{figure}[!ht]
\hskip -0.5cm\begin{minipage}{0.53\textwidth}
\centering
\begin{tabular}{c}
\includegraphics[width=0.8\columnwidth]{figs/error_epoch_reduction.pdf}\\
\end{tabular}
\caption{Test error vs.\ %number of 
epoch reduction in CIFAR10 \& ImageNet training. 
%The 
Dashed lines are test errors of %the 
SGD.
%baseline. 
For CIFAR, SRSGD 
%training 
with fewer epochs can achieve comparable results to SRSGD 
%training 
with 
%full 
200 epochs. For ImageNet, training with less epochs slightly decreases the performance of SRSGD but still achieves comparable results to the SGD baseline.}% training.}
\label{fig:error-vs-epoch-reduction}
%\end{figure}
\end{minipage}
\hfill\vline\hfill
\hskip 0.2cm\begin{minipage}{0.46\textwidth}
\centering
\begin{tabular}{c}
\includegraphics[width=1.0\columnwidth]{figs/ablation_restarting_frequency.pdf}\\
\end{tabular}
\caption{Training loss and test error of Pre-ResNet-290 trained on CIFAR10 with different initial restarting frequencies $F_1$ (linear schedule). SRSGD with small $F_1$ approximates SGD without momentum, while SRSGD with large $F_1$ approximates NASGD.}
\label{fig:ablation_restarting_frequency}
%\end{figure}
\end{minipage}
\vskip -0.5cm
\end{figure}

%\subsection{Impact of Restarting Frequency}
\paragraph{Impact of Restarting Frequency}
We examine the impact of restarting frequency on the network training. We choose a case study of training Pre-ResNet-290 on CIFAR10 using SRSGD with a linear schedule scheme for the restarting frequency. We fix the growth rate $r=2$ and vary the initial restarting frequency $F_{1}$ from 1 to 80 in increments of 10. As shown in Fig.~\ref{fig:ablation_restarting_frequency},  SRSGD with large $F_{1}$, e.g. $F_{1}=80$, approximates NASGD (yellow). As discussed in Section~\ref{section:SRSGD}, it suffers from error accumulation due to stochastic gradients and converges slowly. SRSGD with small $F_{1}$, e.g. $F_{1}=1$, approximates SGD without momentum (green). It converges faster initially but reaches a worse local minimum (i.e. greater loss). Typical SRSGD (blue) converges faster than NASGD and to a better local minimum than both NASGD and SGD without momentum. It also achieves the best test error. We provide more results in Appendix~\ref{sec:impact-restarting-frequency-appendix} and~\ref{appendix:FullTrainingLessEpochs}.





==> sections/intro.tex <==
Training many machine learning (ML) models reduces to solving the following 
%finite-sum 
optimization problem
{\small \begin{equation}
\label{eq:finite-sum}
\min_\vw f(\vw) := \min_\vw \frac{1}{N}\sum_{i=1}^N f_i(\vw),\ \ \vw \in \RR^d,
\end{equation}}
where $f_i(\vw) := \mathcal{L}(g(\bx_i, \vw), y_i)$ is the loss between the ground-truth label $y_i$ and the prediction by the model $g(\cdot, \vw)$, parametrized by $\vw$. This training loss is typically a cross-entropy loss for classification and a root mean square error for regression. Here $\{\bx_i, y_i\}_{i=1}^N$ are the training samples, and problem \eqref{eq:finite-sum} is known as {\em empirical risk minimization} (ERM). For many practical applications, $f(\vw)$ is highly non-convex, and $g(\cdot, \vw)$ is chosen among deep neural networks (DNNs) due to their preeminent performance across various tasks. These deep models are heavily overparametrized and require large amounts of training data. Thus, both $N$ and the dimension of $\vw$ can scale up to millions or even billions. These complications pose serious computational challenges.

One of the simplest algorithms to solve 
%an ERM such as 
\eqref{eq:finite-sum} is gradient descent (GD), which updates $\vw$ according to:
{\small \begin{equation}
\label{eq:GD}
\vw^{k+1} = \vw^k - s_k\frac{1}{N}\sum_{i=1}^N\nabla f_i(\vw^k),
\end{equation}}
where $s_k > 0$ is the step size at the $k$-th iteration. Computing $\nabla f(\vw^k)$ on the entire training set is memory intensive and often cannot fit on devices with limited random access memory (RAM) such as graphics processing units (GPUs) typically used for deep learning (DL). In practice, we 
%instead randomly 
sample a 
%small 
subset of 
%$[N] := \{1, 2, \cdots, N\}$ 
the training set, 
of size $m$ with $m\ll N$, 
%, where $[N]\doteq \{1, 2, \cdots, N\}$, 
to approximate $\nabla f(\vw^k)$ by the mini-batch gradient $1/m\sum_{j=1}^m \nabla f_{i_j}(\vw^k)$. This results in the stochastic gradient descent (SGD) update
{\small \begin{equation}
\label{eq:SGD}
\vw^{k+1} = \vw^k - s_k\frac{1}{m}\sum_{j=1}^m\nabla f_{i_j}(\vw^k).
\end{equation}}
SGD and its accelerated variants are among the most used optimization algorithms in ML practice \cite{bottou2018optimization}. These gradient-based algorithms have a number of benefits. Their convergence rate is usually independent of the dimension of the underlying problem \cite{bottou2018optimization}; their computational complexity is low and easy to parallelize, which makes them suitable to large scale and high dimensional problems \cite{zinkevich2010parallelized,zhang2015deep}. They have achieved, so far, the best performance in training %modern many ML models, in particular, 
 DNNs \cite{goodfellow2016deep}.

Nevertheless, GD and SGD have convergence issues, especially when the problem is ill-conditioned. There are two common approaches to accelerate GD:
%in ill-conditioned scenarios: 
adaptive step size \cite{duchi2011adaptive,hinton2012neural,zeiler2012adadelta} and momentum \cite{polyak1964some}. 
%The integration of both adaptive step size and momentum with SGD is widely used in training DNNs \cite{kingma2014adam,reddi2019convergence,dozat2016incorporating,loshchilov2018fixing,liu2019variance}.
The integration of both adaptive step size and momentum with SGD leads to Adam \cite{kingma2014adam}, which is one of the most used optimizers for DNNs. Many recent developments have improved Adam \cite{reddi2019convergence,dozat2016incorporating,loshchilov2018fixing,liu2020on}. 
GD with constant momentum leverages previous step 
%information 
to accelerate GD according to:
{\small \begin{eqnarray}
\label{eq:ConstanMomentum}
\begin{aligned}
  \vv^{k+1} &= \vw^k -  s_k\nabla f(\vw^k),\\
  \vw^{k+1} &= \vv^{k+1} + \mu (\vv^{k+1} - \vv^{k}),
\end{aligned}
\end{eqnarray}}
where $\mu > 0$ is a constant.
%, without cause ambiguity, we call this weight parameter as momentum. 
A similar acceleration can be achieved by the heavy-ball (HB) method \cite{polyak1964some}. Both momentum update in \eqref{eq:ConstanMomentum} and HB enjoy the same convergence rate of $O(1/k)$ as GD for convex smooth optimization. A breakthrough due to Nesterov \cite{nesterov1983method} replaces the constant momentum $\mu$ with $(k-1)/(k+2)$ (aka, Nesterov accelerated gradient (NAG) momentum), and it can accelerate the convergence rate to $O(1/k^2)$, which is optimal for convex and smooth loss functions \cite{nesterov1983method,su2014differential}. Jin et al. showed that NAG can also speed up escaping saddle point  \cite{jin2017accelerated}. In practice, NAG momentum and its variants such as Katyusha momentum \cite{allen2017katyusha} can also accelerate GD for  nonconvex optimization, especially when the underlying loss function is poorly conditioned \cite{goh2017momentum}.

However, Devolder et al. \cite{devolder2014first} has recently showed that NAG accumulates error when an inexact gradient
%oracle such as stochastic gradient 
is used.
%, thereby slowing convergence at best and diverging at worst. 
Until now, only constant momentum has been successfully used in training DNNs in practice \cite{sutskever2013importance}. Since NAG momentum has achieved a much better convergence rate than constant momentum methods with exact gradient oracle, in this paper we study the following question:

\emph{Can we leverage NAG momentum to accelerate SGD and to improve %convergence and 
generalization in training DNNs?}

\paragraph{Contributions.}
We answer the above question by proposing the first algorithm that integrates scheduled restart (SR) NAG momentum with plain SGD. 
%to accelerate training DNNs. 
We name the resulting algorithm scheduled restart SGD (SRSGD). \emph{Theoretically, we present the %divergence 
error accumulation of Nesterov accelerated SGD (NASGD) and the convergence of SRSGD.} The major practical benefits of SRSGD are fourfold:
\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
    \item SRSGD can significantly speed up DNN training. For image classification, SRSGD can \emph{significantly reduce the number of training epochs while preserving or even improving the network's accuracy}. In particular, on CIFAR10/100, the number of training epochs can be reduced by half with SRSGD while on ImageNet the reduction in training epochs is also remarkable.
    %ranges from 10 to 30 and increases with the network's depth.
    \vspace{0.05in}
    \item DNNs trained by SRSGD \emph{generalize significantly better} than the current benchmark optimizers. 
    %those trained by SGD with constant momentum. 
     \vspace{0.05in}
    \emph{The improvement becomes more significant as the network grows deeper} as shown in Fig.~\ref{fig:error-vs-depth}. 
    \item SRSGD \emph{reduces overfitting in very deep networks} such as ResNet-200 for ImageNet classification, enabling the accuracy to keep increasing with depth.
    \vspace{0.05in}
    \item SRSGD is \emph{straightforward to implement} and only requires changes in a few lines of the SGD code. There is also no additional computational or memory overhead.
\end{itemize}
%To the best of our knowledge, our paper is the first study of NAG momentum with scheduled restart to accelerate SGD for training DNNs. 
We focus on DL for image classification, in which SGD with constant momentum is the 
%common 
choice. 

\begin{figure*}[t!]
\centering
\includegraphics[width=0.7\linewidth]{figs/error_vs_depth_srsgd.pdf}
\vskip -0.3cm
\caption{Error vs. depth of ResNet models trained with SRSGD and the baseline SGD with constant momemtum. Advantage of SRSGD continues to grow with depth.}
\label{fig:error-vs-depth}
\end{figure*}

\paragraph{Organization.}
In Section~\ref{section:momentum}, we review and discuss 
momentum 
for accelerating GD in convex smooth optimization. In Section~\ref{section:SRSGD}, we present 
%scheduled restart NAG momentum to accelerate SGD, namely 
SRSGD algorithm and its theoretical guarantees. In Section~\ref{section:experiments}, we verify the efficacy of the proposed SRSGD in training DNNs for image classification on CIFAR and ImageNet. In Section~\ref{section:Empirical-Analysis}, we perform some empirical analysis of SRSGD. In Section~\ref{section:related_work}, we briefly review some 
%more 
representative works that utilize momentum to accelerate SGD and study the restart techniques in NAG. We end with concluding remarks. Technical proofs and some more experimental details and results, in particular training RNNs and GANs, are provided in the appendix.

\paragraph{Notation.}
We denote scalars and vectors by lower case and lower case bold face letters, resp.,
%vectors by lower case bold face letters, 
and matrices by upper case bold face letters. For a vector $\vx = (x_1, \cdots, x_d)\in \mathbb{R}^d$, we denote its $\ell_p$ norm ($p\geq 1$) 
%of $\vx$ 
by $\|\vx\|_p = {\small \left(\sum_{i=1}^d |x_i|^p\right)^{1/p}}$.
%, the $\ell_\infty$ norm of $\vx$ by $\|\vx\|_\infty = \max_{i=1}^d|x_i|$. 
For a matrix $\Ab$, we used $\|\Ab\|_p$ to denote its induced norm by the vector $\ell_p$ norm. Given two sequences $\{a_n\}$ and $\{b_n\}$, we write $a_n=O(b_n)$ if there exists 
a positive constant s.t.
%$0<C<+\infty$ 
%such that 
$a_n \leq C b_n$. We denote the interval $a$ to $b$ (included) as $(a, b]$. 
%we denote the set $\{1, 2, \cdots, m\}$ as $[m]$.
For a function $f(\vw): \mathbb{R}^d \rightarrow \mathbb{R}$, we denote its gradient and Hessian as $\nabla f(\vw)$ and $\nabla^2 f(\vw)$, respectively.

==> sections/momentum_in_GD.tex <==
%\subsection{Gradient Descent}
%\paragraph{Gradient Descent.} 
\paragraph{GD.} Perhaps the simplest algorithm to solve \eqref{eq:finite-sum} is GD \eqref{eq:GD}, which dates back to \cite{cauchy1847methode}.
%, and it is given in . 
If 
%the objective 
$f(\vw)$ is convex and $L$-smooth (i.e., $\|\nabla^2 f(\vw)\|_2\leq L$), then GD converges with rate $O(1/k)$ by letting $s_k \equiv 1/L$ (we use this $s_k$ in all the discussion below), which is independent of the dimension of $\vw$.

%\subsection{Gradient Descent with Momentum}
\paragraph{HB.} %We can accelerate GD by the 
HB scheme \eqref{eq:HeavyBall} \cite{polyak1964some} accelerates GD by using the momentum $\vw^k - \vw^{k-1}$, which gives
\vskip -0.5cm
{\small \begin{equation}
\label{eq:HeavyBall}
\vw^{k+1} = \vw^k - s_k\nabla f(\vw^k) + \mu (\vw^k - \vw^{k-1}),\ \ \mu >0.
\end{equation}}
%where $\mu > 0$ is a constant. 
Alternatively, we can accelerate GD by using the Nesterov  momentum (aka, lookahead momentum), which leads to 
%the scheme in 
\eqref{eq:ConstanMomentum}. Both HB and 
%the lookahead momentum in 
\eqref{eq:ConstanMomentum} have the same convergence rate of $O(1/k)$ for solving convex smooth problems. Recently, several variants of \eqref{eq:ConstanMomentum}
have been proposed for DL, 
e.g., \cite{sutskever2013importance} and \cite{bengio2013advances}. 

%\subsection{Nesterov Accelerated Gradient}
%\paragraph{Nesterov Accelerated Gradient.}
\paragraph{NAG.}
%\emph{Nesterov accelerated gradient} (NAG) 
NAG \cite{nesterov1983method,beck2009fast} replaces 
%the constant 
$\mu$ with $(t_k-1)/t_{k+1}$, where $t_{k+1}=(1+\sqrt{1+4t_k^2})/2$ with $t_0=1$, 
%with $(k-1)/(k+2)$ or $(k-1)/(k+n)$ for any integer $n\geq 2$,\footnote{This is taken from \cite{su2014differential}.} 
%resulting in
\vskip -0.5cm
{\small \begin{eqnarray}
\label{eq:NAG}
\begin{aligned}
  \vv^{k+1} &= \vw^k -  s_k\nabla f(\vw^k),\\
  \vw^{k+1} &= \vv^{k+1} + \frac{t_k-1}{t_{k+1}} (\vv^{k+1} - \vv^{k}).
\end{aligned}
\end{eqnarray}}
%This is called the \emph{Nesterov accelerated gradient} (NAG) scheme. 
NAG achieves a convergence rate $O(1/k^2)$ with the step size $s_k=1/L$. 
%With the same step size as GD, NAG achieves a convergence rate $O(1/k^2)$, which is the optimal rate for general convex smooth optimization problems.

\begin{remark}
Su et al. \cite{su2014differential} showed that $(k-1)/(k+2)$ is the asymptotic limit of $(t_k-1)/t_{k+1}$. In the following presentation of NAG with restart, for the ease of notation, we will replace the momentum coefficient $(t_k-1)/t_{k+1}$ with the form of $(k-1)/(k+2)$.
\end{remark}

%\subsection{Adaptive Restart NAG}
\paragraph{Adaptive Restart NAG (ARNAG).} 
%Consider the sequence $\{f(\vw_k)-f(\vw^*)\}$ where $\vw^*$ is the minimum of $f(\vw)$. 
The sequences, $\{f(\vw^k)-f(\vw^*)\}$ where $\vw^*$ is the minimum of $f(\vw)$, generated by GD and GD with constant momentum (GD $+$ Momentum) converge monotonically to zero. However, that sequence generated by NAG oscillates, 
%to zero in an oscillatory way, 
as illustrated in Fig.~\ref{fig:Quadratic-Compare-Optimization} (a) 
when $f(\vw)$ is a quadratic function.
%ARNAG \eqref{eq:ARNAG} 
\cite{o2015adaptive} proposes ARNAG \eqref{eq:ARNAG} to alleviate this oscillatory phenomenon
%adaptive restart NAG 
%(ARNAG) 
%\cite{o2015adaptive}
\vskip -0.5cm
{\small \begin{eqnarray}
\label{eq:ARNAG}
\begin{aligned}
  \vv^{k+1} &= \vw^k -  s_k\nabla f(\vw^k),\\
  \vw^{k+1} &= \vv^{k+1} + \frac{m(k)-1}{m(k)+2} (\vv^{k+1} - \vv^{k}),
\end{aligned}
\end{eqnarray}}
where $m(1)=1$; $m(k+1)=m(k)+1$ if $f(\vw^{k+1}) \leq f(\vw^{k})$, and $m(k+1)=1$ otherwise. 
%{\small $$
%m_k = \begin{cases}
%t_k,\ \ &\mbox{if}\ \ f(\vw^k) \leq f(\vw^{k-1}),\\
%1, & \mbox{otherwise.}
%\end{cases}
%$$}
%Roulet et al. \cite{roulet2017sharpness} 
%showed that 
%, under sharpness assumption, 
%AR accelerates NAG to linear convergence for convex problems with sharpness assumption \cite{roulet2017sharpness}.
%rate in certain circumstances.


%\subsection{Scheduled Restart NAG} \label{sec:SRNAG}
\paragraph{Scheduled Restart NAG (SRNAG).} \label{sec:SRNAG}
SR is another strategy to restart NAG. 
We first divide the total iterations $(0, T]$ (integers only) into a few intervals $\{I_i\}_{i=1}^m = (T_{i-1}, T_i]$, such that $(0, T] = \bigcup_{i=1}^m I_i$. In each $I_i$ we restart the momentum after every $F_i$, and the iteration is according to:
%iterations as follows:
{\small \begin{eqnarray}
\label{eq:SRNAG}
\begin{aligned}
  \vv^{k+1} &= \vw^k -  s_k\nabla f(\vw^k),\\
  \vw^{k+1} &= \vv^{k+1} + \frac{(k\bmod F_i)}{(k\bmod F_i) + 3} (\vv^{k+1} - \vv^{k}).
\end{aligned}
\end{eqnarray}}
%Again, Roulet et al. \cite{roulet2017sharpness} showed that, under an extra sharpness assumption, 
Both AR and SR accelerate NAG to linear convergence for convex problems with PL 
%sharpness 
condition \cite{roulet2017sharpness}.


%\subsection{Case Study -- Quadratic Function}
\paragraph{Case Study -- Quadratic Function.}
Consider the following quadratic optimization\footnote{We take this example from \cite{mrtz}.}
{\small \begin{equation}\label{eq:quadratic}
\min_\vx f(\vx) = \frac{1}{2}\vx^T\mathbf{L}\vx - \vx^T\vb,
\end{equation}}
where $\mathbf{L} \in \mathbb{R}^{d\times d}$ is the Laplacian of a cycle graph.
%$$
%\mathbf{L} = 
%\begin{pmatrix}
%     2&-1&0&\cdots&0&-1  \\
%     -1&2&-1&0&\cdots&0  \\
%     \cdots & \cdots & \cdots & \cdots & \cdots & \cdots \\
%     0&\cdots&0&-1&2&-1\\
%     -1&0&\cdots&0&-1&2\\
%\end{pmatrix}_{d\times d}$$
and $\vb$ is a $d$-dimensional vector whose first entry is $1$ and all the other entries are $0$. It is easy to see that $f(\vx)$ is convex with Lipschitz constant $4$. In particular, we set $d=1$K ($1$K$ := 10^3$). We run $T=50$K iterations with step size $1/4$. In SRNAG, we restart, i.e., we set the momentum to 0, after every $1$K iterations. 
As shown in Fig.~\ref{fig:Quadratic-Compare-Optimization} (a), GD $+$ Momentum converges faster than GD, while NAG speeds up GD $+$ Momentum dramatically and converges to the minimum in an oscillatory fashion. Both AR and SR accelerate NAG significantly.


\begin{figure*}[!ht]
\centering
\includegraphics[width=0.7\linewidth]{figs/quadratic.pdf}
\vskip -0.3cm
\caption{Comparison between different schemes in optimizing the quadratic function, 
%$f(\vx)$ in 
\eqref{eq:quadratic}, with (a) exact gradient, (b) gradient with constant variance Gaussian noise, and (c) gradient with decaying variance Gaussian noise. NAG, ARNAG, and SRNAG can speed up convergence remarkably when exact gradient is used. %However, 
Also, SRNAG is more robust to noisy gradient than NAG and ARNAG.
}
\label{fig:Quadratic-Compare-Optimization}
\end{figure*}

==> sections/related_work.tex <==
\begin{comment}
\begin{figure}[!t]
\centering
\includegraphics[width=1.0\linewidth]{figs/ablation_restarting_frequency.pdf}
\caption{Training loss and test error of Pre-ResNet-290 trained on CIFAR10 with different initial restarting frequencies $F_1$ (linear schedule). SRSGD with small $F_1$ approximates SGD without momentum, while SRSGD with large $F_1$ approximates NASGD.}
\label{fig:ablation_restarting_frequency}
\end{figure}
\end{comment}

Momentum has long been used to accelerate SGD. \cite{sutskever2013importance} showed that SGD with scheduled momentum and a %well-designed 
good initialization can handle 
%deal with 
the curvature issues in training DNNs and enable the trained models to generalize well. \cite{kingma2014adam,dozat2016incorporating} integrated momentum with adaptive step size to accelerate SGD. These works all leverage constant momentum, while our work utilizes NAG momentum with restart. AR and SR have been used to accelerate NAG with exact gradient \cite{nemirovskii1985optimal,nesterov2013gradient,iouditski2014primal,lin2014adaptive,renegar2014efficient,freund2018new,roulet2015computational,o2015adaptive,giselsson2014monotonicity,su2014differential}. These studies of restart NAG momentum are for convex optimization with exact gradient. Our work focuses on SGD for nonconvex optimization.  Many efforts have also been devoted to accelerating first-order algorithms with noise-corrupted gradients \cite{cohen2018acceleration,aybat2018robust}.

==> sections/srsgd.tex <==
Computing 
%exact 
gradient for 
%the
ERM, \eqref{eq:finite-sum}, can be computational costly and memory intensive, especially when the training set is large. In many 
%practical 
applications, such as training DNNs, 
%the SGD update in \eqref{eq:SGD} 
SGD \eqref{eq:SGD} is used. 
%instead. 
In this section, we will first analyze whether NAG and restart techniques can still speed up SGD.
%convergence when stochastic gradient or other types of inexact gradient are used. 
Then we formulate our new SRSGD as a solution to accelerate convergence of SGD using NAG momentum.
%in SGD.
%inexact oracle settings, which includes SGD update.

\subsection{Uncontrolled Bound of Nesterov Accelerated SGD (NASGD)}
%\subsection{Divergence of NASGD}
Replacing {\small$\nabla f(\vw^k) :=1/N\sum_{i=1}^N\nabla f_i(\vw^k)$} in \eqref{eq:NAG} with the stochastic gradient {\small$1/m\sum_{j=1}^m\nabla f_{i_j}(\vw^k)$} for \eqref{eq:finite-sum} will accumulate error even for convex function. We formulate this fact in Theorem~\ref{Theorem:divergence-NASGD-Main}.
%, the proof is provided in the appendix.

\begin{theorem}
\label{Theorem:divergence-NASGD-Main}
Let $f(\vw)$ be a convex and $L$-smooth function. The sequence $\{\vw^k\}_{k\geq 0}$ generated by \eqref{eq:NAG}, with mini-batch stochastic gradient using any constant step size $s_k \equiv s \leq 1/L$, satisfies
\begin{equation}
\label{eq:divergence:NASGD-result}
{\small \mathbb{E}\left(f(\vw^k)-f(\vw^*)\right) = O(k),}
\end{equation}
where $\vw^*$ is the minimum of $f$, and the expectation is taken over the random mini-batch samples.
\end{theorem}

%NAG momentum not only accumulates error in SGD, but also accumulates error in the $\delta$-inexact gradient \cite{devolder2014first}. A similar error accumulation rate was established in \cite{devolder2014first}. 
%The proof of Theorem~\ref{Theorem:divergence-NASGD-Main} is given in Appendix~A. 
In Appendix~\ref{appendix:uncontrolled:NASGD}, we provide the proof of Theorem~\ref{Theorem:divergence-NASGD-Main}. %Appendix~A.
In \cite{devolder2014first}, Devolder et al. proved a similar error accumulation result for the $\delta$-inexact gradient. In Appendix~\ref{appendix:Delta:Inexact:Gradient}, we provide a brief review of NAG with $\delta$-inexact gradient. We consider three different inexact gradients, namely, Gaussian noise with constant and decaying variance corrupted gradients for the quadratic optimization \eqref{eq:quadratic}, and training logistic regression model for MNIST \cite{lecun-mnisthandwrittendigit-2010} classification. The detailed settings and discussion are provided in the Appendix~~\ref{appendix:Delta:Inexact:Gradient}. We denote SGD with NAG momentum as NASGD, and denote NASGD with AR and SR as ARSGD and SRSGD, respectively. The results shown in Fig.~\ref{fig:Quadratic-Compare-Optimization} (b) and (c) (iteration vs.\ optimal gap for quadratic optimization \eqref{eq:quadratic}
%, $f(\vx^k) - f(\vx^*)$ with $\vx^*$ being the minimum
), and Fig.~\ref{fig:Logistic-Regression-Comparison} (iteration vs. loss for training logistic regression model) confirm Theorem~\ref{Theorem:divergence-NASGD-Main}. Moreover, for these cases SR can improve the performance of NAG with inexact gradients. %This motivates us to leverage NAG momentum with SR to accelerate SGD, which leads to SRSGD. 
%, which is applicable to highly non-convex non-smooth problem such as training DNNs.
When inexact gradient is used, GD performs almost the same as ARNAG asymptotically because ARNAG restarts too often and almost degenerates to GD. 



%Based on the results from our case study, we conclude that SR can improve the performance of NAG with inexact gradients. This motivates us to leverage NAG momentum with scheduled restart to accelerate SGD, which leads to our SRSGD method, which is applicable to highly non-convex non-smooth problem such as training DNNs.

\begin{figure}[!ht]
\begin{minipage}{0.48\textwidth}
\centering
\begin{tabular}{c}
\includegraphics[width=0.65\columnwidth]{figs/regression.pdf}\\
\end{tabular}
\vskip -0.3cm
\caption{Training loss comparison between different schemes in training logistic regression for MNIST classification. NASGD is not robust to noisy gradient, ARSGD almost degenerates to SGD, and SRSGD performs the best in this case.}
\label{fig:Logistic-Regression-Comparison}
%\end{figure}
\end{minipage}
\hfill\vline\hfill
\begin{minipage}{0.5\textwidth}
%\begin{figure}[H]
\centering
\begin{tabular}{c}
\includegraphics[width=1.0\columnwidth]{figs/train_loss_vs_epoch_srsgd.pdf}\\
\end{tabular}
\caption{Training loss vs. training epoch of ResNet models trained with SRSGD (blue) and the SGD baseline with momentum (red).}
\label{fig:train-loss-vs-epoch}
\end{minipage}
\vskip -0.3cm
\end{figure}




\begin{comment}
\begin{minipage}{0.4\textwidth}
\begin{figure}[H]
\centering
\begin{tabular}{c}
\includegraphics[width=0.9\columnwidth]{figs/regression.pdf}\\
\end{tabular}
\caption{Training loss comparison between different schemes in training logistic regression for MNIST classification. NASGD is not robust to noisy gradient, ARSGD almost degenerates to SGD, and SRSGD performs the best in this case.}
\label{fig:Logistic-Regression-Comparison}
\end{figure}
\end{minipage}
\hfill
\begin{minipage}{0.55\textwidth}
\begin{figure}[H]
\centering
\begin{tabular}{c}
\includegraphics[width=0.9\columnwidth]{figs/regression.pdf}\\
\end{tabular}
\caption{Training loss comparison between different schemes in training logistic regression for MNIST classification. NASGD is not robust to noisy gradient, ARSGD almost degenerates to SGD, and SRSGD performs the best in this case.}
\label{fig:Logistic-Regression-Comparison}
\end{figure}
\end{minipage}
\end{comment}




\subsection{SRSGD and Its Convergence}\label{subsection:SRSGD}
%We now formulate SRSGD. Considering the finite-sum optimization in \eqref{eq:finite-sum}, 
%Consider solving 
For ERM \eqref{eq:finite-sum}, SRSGD replaces $\nabla f(\vw)$ in \eqref{eq:SRNAG} with the stochastic gradient with batch size $m$, gives
%resulting in
{\small \begin{eqnarray}
\label{eq:SRSGD}
\begin{aligned}
  \vv^{k+1} &= \vw^k -  s_k\frac{1}{m}\sum_{j=1}^m\nabla f_{i_j}(\vw^k),\\
  \vw^{k+1} &= \vv^{k+1} + \frac{(k\bmod F_i)}{(k\bmod F_i) + 3} (\vv^{k+1} - \vv^{k}),
\end{aligned}
\end{eqnarray}}
where $F_i$ is the restart frequency used in the interval $I_i$. 
%$F_i$ and $I_i$ are previously defined in~\ref{sec:SRNAG}.
%\emph{SRSGD leverages NAG-style momentum to accelerate SGD}, and we 
We implemented SRSGD in both PyTorch \cite{paszke2019pytorch} and Keras \cite{chollet2015keras}, by changing just a few lines on top of the existing SGD 
%with momentum 
optimizer. We provide a snippet of SRSGD code in Appendix~\ref{appendix:PyTorch} and \ref{appendix:Keras}. We formulate the convergence of SRSGD for general 
%convex or 
nonconvex problems 
%is given 
in Theorem~\ref{Theorem:convergence:SRSGD:main} and we provide its proof in Appendix~\ref{appendix:Convergence:SRSGD}.

\begin{theorem}
\label{Theorem:convergence:SRSGD:main}
Suppose $f(\vw)$ is $L$-smooth. Consider the sequence $\{\vw^k\}_{k\geq 0}$ generated by \eqref{eq:SRSGD} with mini-batch stochastic gradient and any restart frequency $F$ using any constant step size $s_k := s\leq 1/L$. Assume that the set $\mathcal{A} := \{k\in \mathbb{Z}^+| \mathbb{E}f(\vw^{k+1})\geq \mathbb{E}f(\vw^k) \}$ is finite, then we have 
{\small \begin{equation}
\label{eq:convergence:SRSGD}
\min_{1\leq k\leq K}\left\{\mathbb{E}\|\nabla f(\vw^k)\|_2^2\right\} = O(s+ \frac{1}{sK}).
\end{equation}}
Therefore for $\forall \epsilon>0$, to get $\epsilon$ error, we just need to set $s=O(\epsilon)$ and $K=O(1/\epsilon^2)$.
\end{theorem}
